EXPRES IV: Two Additional Planets Orbiting $\rho$ Coronae Borealis Reveal Uncommon System Architecture

Thousands of exoplanet detections have been made over the last twenty-five years using Doppler observations, transit photometry, direct imaging, and astrometry. Each of these methods is sensitive to different ranges of orbital separations and planetary radii (or masses). This makes it difficult to fully characterize exoplanet architectures and to place our solar system in context with the wealth of discoveries that have been made. Here, we use the EXtreme PREcision Spectrograph (EXPRES) to reveal planets in previously undetectable regions of the mass-period parameter space for the star $\rho$ Coronae Borealis. We add two new planets to the previously known system with one hot Jupiter in a 39-day orbit and a warm super-Neptune in a 102-day orbit. The new detections include a temperate Neptune planet ($M{\sin{i}} \sim 20$ M$_\oplus$) in a 281.4-day orbit and a hot super-Earth ($M{\sin{i}} = 3.7$ M$_\oplus$) in a 12.95-day orbit. This result shows that details of planetary system architectures have been hiding just below our previous detection limits; this signals an exciting era for the next generation of extreme precision spectrographs.

==> expres_rvs_full.tex <==
\begin{deluxetable}{ccc}
\tablecaption{EXPRES RVs of HD 143761 \label{tab:143761vels}}
\tablehead{\colhead{BMJD} & \colhead{Vel \ms} & \colhead{Err \ms}}
\startdata
58983.23654927 & 28.913 & 0.420 \\
58983.23864388 & 29.743 & 0.438 \\
58983.24077284 & 27.107 & 0.445 \\
59012.37000357 & 52.129 & 0.445 \\
59012.37211914 & 54.251 & 0.445 \\
59012.37400430 & 54.915 & 0.458 \\
59017.30889883 & 59.608 & 0.419 \\
59335.41151111 & 58.781 & 0.377 \\
59335.41464020 & 58.331 & 0.378 \\
59335.41764142 & 58.228 & 0.372 \\
59336.37561661 & 55.901 & 0.337 \\
59336.38102249 & 55.415 & 0.343 \\
59339.40019249 & 37.521 & 0.342 \\
59339.40549467 & 37.177 & 0.357 \\
59356.41524095 & -68.069 & 0.355 \\
59358.41265226 & -61.742 & 0.343 \\
59360.39906687 & -46.917 & 0.357 \\
59361.40085295 & -35.163 & 0.350 \\
59361.40498701 & -36.474 & 0.350 \\
59364.39615719 & -3.037 & 0.360 \\
59364.39926398 & -0.935 & 0.382 \\
59365.42032061 & 11.380 & 0.407 \\
59366.34199547 & 22.596 & 0.397 \\
59366.34464072 & 21.485 & 0.408 \\
59378.21191614 & 55.569 & 0.357 \\
59378.21520880 & 55.140 & 0.347 \\
59381.25066476 & 31.157 & 0.380 \\
59381.25552548 & 32.336 & 0.393 \\
59383.26143550 & 11.846 & 0.476 \\
59385.23453173 & -7.928 & 0.442 \\
59385.24353940 & -9.164 & 0.423 \\
59413.26280320 & 64.067 & 0.531 \\
59413.27510384 & 65.511 & 0.467 \\
59434.17787081 & -68.961 & 0.407 \\
59434.18099128 & -68.556 & 0.426 \\
59447.13734138 & 30.732 & 0.362 \\
59447.14210657 & 31.804 & 0.427 \\
59448.13237941 & 39.176 & 0.375 \\
59448.13508356 & 38.806 & 0.355 \\
59449.13443902 & 46.671 & 0.383 \\
59449.13719307 & 45.645 & 0.343 \\
59450.12291678 & 56.058 & 0.395 \\
59450.12562862 & 54.273 & 0.366 \\
59451.14114198 & 60.377 & 0.398 \\
59451.14414288 & 59.891 & 0.404 \\
59466.10944977 & -22.185 & 0.415 \\
59466.11309082 & -19.650 & 0.423 \\
59471.10166536 & -56.574 & 0.392 \\
59471.10505893 & -55.646 & 0.428 \\
59570.54888304 & 58.375 & 0.354 \\
59570.55243954 & 59.567 & 0.388 \\
59599.48304991 & -41.519 & 0.341 \\
59599.49741811 & -40.686 & 0.371 \\
59603.54626362 & -1.075 & 0.345 \\
59603.54966172 & 0.106 & 0.362 \\
59631.54980046 & -70.051 & 0.350 \\
59651.51828922 & 60.317 & 0.369 \\
59651.52093529 & 59.769 & 0.358 \\
59660.50470085 & 20.848 & 0.337 \\
59660.51385481 & 20.553 & 0.344 \\
59662.40802325 & 2.421 & 0.343 \\
59662.41068556 & 5.130 & 0.340 \\
59665.42024709 & -22.518 & 0.356 \\
59665.42298401 & -22.653 & 0.354 \\
59675.43130943 & -65.673 & 0.338 \\
59675.43476121 & -65.735 & 0.333 \\
59680.47797958 & -28.531 & 0.355 \\
59680.48757952 & -28.304 & 0.359 \\
59682.44574594 & -5.816 & 0.296 \\
59682.45228741 & -7.176 & 0.315 \\
59683.47073224 & 4.463 & 0.333 \\
59683.47388243 & 4.283 & 0.350 \\
59684.45105756 & 17.705 & 0.316 \\
59684.45567678 & 16.792 & 0.363 \\
59686.41121108 & 35.807 & 0.325 \\
59686.41492123 & 34.130 & 0.329 \\
59687.42346373 & 47.079 & 0.351 \\
59687.42719988 & 46.623 & 0.341 \\
59688.45400536 & 57.024 & 0.423 \\
59690.41077091 & 67.377 & 0.366 \\
59690.41501389 & 69.839 & 0.364 \\
59691.38466879 & 70.727 & 0.378 \\
59691.38889089 & 70.319 & 0.388 \\
59701.40942141 & 20.813 & 0.324 \\
59701.41411348 & 21.249 & 0.305 \\
59709.40059574 & -53.026 & 0.367 \\
59709.40561373 & -53.688 & 0.351 \\
59710.39536912 & -58.530 & 0.357 \\
59710.39997182 & -58.245 & 0.354 \\
59712.39469205 & -65.361 & 0.340 \\
59712.39791508 & -66.666 & 0.349 \\
59713.34701416 & -65.878 & 0.316 \\
59713.35067825 & -65.470 & 0.350 \\
59715.39436623 & -64.733 & 0.358 \\
59715.39883003 & -63.479 & 0.373 \\
59716.39550231 & -55.720 & 0.342 \\
59716.40002977 & -57.609 & 0.347 \\
59718.39981620 & -46.797 & 0.370 \\
59718.40788202 & -47.591 & 0.358 \\
59720.31644404 & -30.956 & 0.360 \\
59720.32567438 & -31.819 & 0.387 \\
59721.39307333 & -19.716 & 0.380 \\
59721.39709880 & -15.490 & 0.372 \\
59722.40941023 & -8.302 & 0.362 \\
59722.41564259 & -8.662 & 0.384 \\
59729.22380983 & 56.983 & 0.361 \\
59733.42312375 & 62.484 & 0.363 \\
59736.32361903 & 50.203 & 0.393 \\
59736.32741144 & 49.422 & 0.398 \\
59737.27335870 & 47.774 & 0.372 \\
59737.28089643 & 46.205 & 0.358 \\
59738.39107789 & 38.689 & 0.402 \\
59738.39573449 & 37.832 & 0.407 \\
59740.31701345 & 23.452 & 0.416 \\
59740.32279183 & 21.382 & 0.381 \\
59745.21644726 & -25.240 & 0.346 \\
59745.21995315 & -26.745 & 0.356 \\
59746.23417984 & -36.222 & 0.448 \\
59747.27670672 & -42.238 & 0.401 \\
59979.52832327 & 20.752 & 0.348 \\
59979.53221938 & 24.160 & 0.367 \\
59980.50831775 & 13.563 & 0.357 \\
59980.51198412 & 15.352 & 0.357 \\
60012.51790039 & 69.665 & 0.323 \\
60012.52305212 & 69.029 & 0.343 \\
60013.48627511 & 65.214 & 0.386 \\
60031.50765288 & -67.859 & 0.401 \\
60035.44645984 & -63.621 & 0.365 \\
60035.45588781 & -62.680 & 0.350 \\
60041.49644166 & -4.084 & 0.364 \\
60041.50338241 & -5.217 & 0.358 \\
60046.45968656 & 43.678 & 0.366 \\
60046.46769376 & 43.869 & 0.375 \\
60050.40822257 & 63.224 & 0.343 \\
60050.41191090 & 65.177 & 0.390 \\
60064.42887019 & -31.238 & 0.355 \\
60064.43394611 & -30.873 & 0.373 \\
60066.43256698 & -44.427 & 0.316 \\
60066.44333045 & -44.078 & 0.337 \\
60067.42465836 & -52.602 & 0.367 \\
60067.43037310 & -53.489 & 0.339 \\
60068.43565349 & -59.487 & 0.328 \\
60068.44711451 & -58.071 & 0.329 \\
60069.42482781 & -62.571 & 0.348 \\
60069.42948349 & -64.370 & 0.343 \\
60070.41566273 & -69.313 & 0.346 \\
60070.41930012 & -69.313 & 0.350 \\
60071.42708407 & -71.013 & 0.348 \\
60071.43202362 & -72.196 & 0.329 \\
60072.41770064 & -69.229 & 0.371 \\
60072.42080962 & -70.371 & 0.374 \\
60073.42015155 & -69.476 & 0.351 \\
60073.42375727 & -69.489 & 0.364
\enddata
\end{deluxetable}

